To Ship or Not to Ship: An Extensive Evaluation of Automatic Metrics for Machine Translation

Automatic metrics are commonly used as the exclusive tool for declaring the superiority of one machine translation system's quality over another. The community choice of automatic metric guides research directions and industrial developments by deciding which models are deemed better. Evaluating metrics correlations with sets of human judgements has been limited by the size of these sets. In this paper, we corroborate how reliable metrics are in contrast to human judgements on -- to the best of our knowledge -- the largest collection of judgements reported in the literature. Arguably, pairwise rankings of two systems are the most common evaluation tasks in research or deployment scenarios. Taking human judgement as a gold standard, we investigate which metrics have the highest accuracy in predicting translation quality rankings for such system pairs. Furthermore, we evaluate the performance of various metrics across different language pairs and domains. Lastly, we show that the sole use of BLEU impeded the development of improved models leading to bad deployment decisions. We release the collection of 2.3M sentence-level human judgements for 4380 systems for further analysis and replication of our work.

==> generated/generated_dependent.tex <==
\begin{table}
\centering
\caption{}
\label{tab:dependent}
\begin{tabular}{lll}
\toprule
{} &                          Dependent &                        Independent \\
\midrule
n         &                                161 &                                246 \\
BLEU      &  \cellcolor{black!15}\textbf{99.4} &                               90.7 \\
BERTScore &           \cellcolor{black!15}98.8 &                               91.5 \\
ESIM      &           \cellcolor{black!15}98.8 &                               92.3 \\
COMET     &           \cellcolor{black!15}98.1 &           \cellcolor{black!15}98.4 \\
Prism     &           \cellcolor{black!15}98.1 &                               94.3 \\
ChrF      &           \cellcolor{black!15}98.1 &                               91.5 \\
COMET-src &           \cellcolor{black!15}97.5 &  \cellcolor{black!15}\textbf{98.8} \\
CharacTER &           \cellcolor{black!15}97.5 &                               89.8 \\
BLEURT    &                               96.9 &                               93.5 \\
Prism-src &           \cellcolor{black!15}96.9 &                               92.7 \\
TER       &                               95.7 &                               91.5 \\
EED       &                               78.9 &                               78.0 \\
\bottomrule
\end{tabular}
\end{table}


==> generated/generated_individual_language_pairs.tex <==
\begin{table}
\centering
\caption{}
\label{tab:individual_language_pairs}
\begin{tabular}{llllllllllllll}
\toprule
{} &   n &                               COMET &                           COMET-src &                              BLEURT &                               Prism &                           Prism-src &                                ESIM &                                BLEU &                                ChrF &                           BERTScore &                           CharacTER &                                 TER &                                 EED \\
\midrule
English - French     &  62 &   \cellcolor{black!15}\textbf{98.4} &                                93.5 &                                90.3 &                                88.7 &                                87.1 &                                82.3 &                                64.5 &                                64.5 &                                62.9 &                                62.9 &                                58.1 &                                41.9 \\
Japanese - English   &  58 &   \cellcolor{black!15}\textbf{98.3} &                                89.7 &                                84.5 &   \cellcolor{black!15}\textbf{98.3} &                                89.7 &   \cellcolor{black!15}\textbf{98.3} &                                93.1 &                                93.1 &            \cellcolor{black!15}96.6 &                                87.9 &            \cellcolor{black!15}96.6 &                                82.8 \\
English - Polish     &  57 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}98.2 &  \cellcolor{black!15}\textbf{100.0} &                                82.5 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}98.2 \\
Polish - English     &  55 &                                80.0 &   \cellcolor{black!15}\textbf{98.2} &                                83.6 &                                83.6 &   \cellcolor{black!15}\textbf{98.2} &                                83.6 &                                83.6 &                                80.0 &                                83.6 &                                80.0 &                                81.8 &                                81.8 \\
Thai - English       &  54 &  \cellcolor{black!15}\textbf{100.0} &                                70.4 &            \cellcolor{black!15}96.3 &                                90.7 &                                16.7 &                                88.9 &                                83.3 &                                92.6 &                                90.7 &                                94.4 &                                83.3 &                                20.4 \\
English - German     &  52 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &                                80.8 &  \cellcolor{black!15}\textbf{100.0} &                                88.5 &  \cellcolor{black!15}\textbf{100.0} &                                75.0 &                                67.3 &                                82.7 &                                73.1 &                                78.8 &                                75.0 \\
Chinese - English    &  52 &            \cellcolor{black!15}96.2 &                                94.2 &            \cellcolor{black!15}98.1 &                                92.3 &                                71.2 &  \cellcolor{black!15}\textbf{100.0} &                                94.2 &            \cellcolor{black!15}96.2 &                                94.2 &            \cellcolor{black!15}96.2 &                                86.5 &                                71.2 \\
Turkish - English    &  51 &            \cellcolor{black!15}98.0 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}96.1 &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}96.1 &            \cellcolor{black!15}96.1 &            \cellcolor{black!15}96.1 &            \cellcolor{black!15}96.1 &            \cellcolor{black!15}98.0 &            \cellcolor{black!15}96.1 &                                94.1 \\
English - Indonesian &  51 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}96.1 &  \cellcolor{black!15}\textbf{100.0} &                                88.2 &  \cellcolor{black!15}\textbf{100.0} &                                92.2 &            \cellcolor{black!15}98.0 &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}96.1 &            \cellcolor{black!15}98.0 &            \cellcolor{black!15}96.1 \\
English - Turkish    &  48 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &                                87.5 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}95.8 &                                91.7 \\
English - Swedish    &  48 &                                91.7 &                                91.7 &   \cellcolor{black!15}\textbf{97.9} &   \cellcolor{black!15}\textbf{97.9} &   \cellcolor{black!15}\textbf{97.9} &            \cellcolor{black!15}95.8 &            \cellcolor{black!15}93.8 &                                87.5 &            \cellcolor{black!15}95.8 &            \cellcolor{black!15}95.8 &            \cellcolor{black!15}93.8 &            \cellcolor{black!15}91.7 \\
Swedish - English    &  47 &            \cellcolor{black!15}97.9 &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}97.9 &            \cellcolor{black!15}95.7 &                                89.4 &                                91.5 &                                87.2 &                                91.5 &            \cellcolor{black!15}95.7 &                                72.3 &                                91.5 &                                85.1 \\
English - Dutch      &  47 &            \cellcolor{black!15}97.9 &            \cellcolor{black!15}97.9 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}97.9 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &                                87.2 \\
Indonesian - English &  46 &            \cellcolor{black!15}97.8 &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}97.8 &            \cellcolor{black!15}97.8 &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}97.8 &                                93.5 &            \cellcolor{black!15}97.8 &            \cellcolor{black!15}97.8 &            \cellcolor{black!15}97.8 &                                91.3 &                                89.1 \\
English - Hungarian  &  46 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}97.8 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}97.8 &                                84.8 &                                82.6 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &                                87.0 \\
Czech - English      &  44 &  \cellcolor{black!15}\textbf{100.0} &                                93.2 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &                                93.2 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}95.5 &            \cellcolor{black!15}95.5 &            \cellcolor{black!15}95.5 &                                20.5 \\
English - Czech      &  42 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &                                92.9 &            \cellcolor{black!15}97.6 &            \cellcolor{black!15}97.6 &            \cellcolor{black!15}97.6 &                                92.9 &                                92.9 &            \cellcolor{black!15}97.6 &                                92.9 &            \cellcolor{black!15}97.6 &  \cellcolor{black!15}\textbf{100.0} \\
English - Danish     &  42 &            \cellcolor{black!15}95.2 &            \cellcolor{black!15}95.2 &            \cellcolor{black!15}88.1 &   \cellcolor{black!15}\textbf{97.6} &            \cellcolor{black!15}95.2 &            \cellcolor{black!15}92.9 &   \cellcolor{black!15}\textbf{97.6} &            \cellcolor{black!15}92.9 &            \cellcolor{black!15}95.2 &            \cellcolor{black!15}92.9 &            \cellcolor{black!15}95.2 &                                88.1 \\
Hungarian - English  &  42 &            \cellcolor{black!15}90.5 &                                83.3 &                                78.6 &   \cellcolor{black!15}\textbf{97.6} &                                85.7 &                                90.5 &            \cellcolor{black!15}90.5 &            \cellcolor{black!15}95.2 &                                85.7 &            \cellcolor{black!15}92.9 &                                81.0 &            \cellcolor{black!15}88.1 \\
Hindi - English      &  41 &            \cellcolor{black!15}95.1 &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}95.1 &                                82.9 &                                73.2 &                                78.0 &                                61.0 &                                61.0 &                                80.5 &                                65.9 &                                73.2 &                                80.5 \\
Dutch - English      &  40 &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}97.5 &            \cellcolor{black!15}97.5 &            \cellcolor{black!15}97.5 &                                82.5 &            \cellcolor{black!15}97.5 &            \cellcolor{black!15}97.5 &            \cellcolor{black!15}95.0 &            \cellcolor{black!15}97.5 &            \cellcolor{black!15}97.5 &            \cellcolor{black!15}97.5 &                                75.0 \\
German - English     &  39 &   \cellcolor{black!15}\textbf{97.4} &            \cellcolor{black!15}94.9 &   \cellcolor{black!15}\textbf{97.4} &   \cellcolor{black!15}\textbf{97.4} &                                82.1 &            \cellcolor{black!15}94.9 &                                82.1 &                                82.1 &   \cellcolor{black!15}\textbf{97.4} &                                82.1 &            \cellcolor{black!15}94.9 &                                64.1 \\
Danish - English     &  39 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}97.4 &            \cellcolor{black!15}97.4 &  \cellcolor{black!15}\textbf{100.0} &                                89.7 &            \cellcolor{black!15}97.4 &                                74.4 \\
Spanish - English    &  39 &            \cellcolor{black!15}94.9 &            \cellcolor{black!15}94.9 &            \cellcolor{black!15}94.9 &   \cellcolor{black!15}\textbf{97.4} &            \cellcolor{black!15}92.3 &            \cellcolor{black!15}94.9 &            \cellcolor{black!15}94.9 &            \cellcolor{black!15}94.9 &   \cellcolor{black!15}\textbf{97.4} &   \cellcolor{black!15}\textbf{97.4} &            \cellcolor{black!15}94.9 &            \cellcolor{black!15}92.3 \\
English - Russian    &  37 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &                                91.9 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} \\
Portuguese - English &  36 &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}94.4 &            \cellcolor{black!15}94.4 &            \cellcolor{black!15}94.4 &            \cellcolor{black!15}94.4 &            \cellcolor{black!15}94.4 &            \cellcolor{black!15}94.4 &                                88.9 &            \cellcolor{black!15}94.4 &            \cellcolor{black!15}94.4 &            \cellcolor{black!15}94.4 &            \cellcolor{black!15}97.2 \\
Korean - English     &  33 &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}97.0 &                                72.7 &                                87.9 &                                42.4 &                                69.7 &                                63.6 &            \cellcolor{black!15}97.0 &                                78.8 &                                90.9 &                                69.7 &                                66.7 \\
English - Portuguese &  31 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &                                87.1 &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}96.8 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}96.8 &  \cellcolor{black!15}\textbf{100.0} \\
English - Italian    &  28 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}96.4 &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}96.4 &            \cellcolor{black!15}96.4 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}96.4 &                                75.0 \\
English - Japanese   &  28 &            \cellcolor{black!15}96.4 &                                89.3 &  \cellcolor{black!15}\textbf{100.0} &            \cellcolor{black!15}96.4 &                                75.0 &            \cellcolor{black!15}96.4 &                                78.6 &            \cellcolor{black!15}96.4 &            \cellcolor{black!15}96.4 &                                67.9 &                                78.6 &                                46.4 \\
Russian - English    &  27 &            \cellcolor{black!15}92.6 &  \cellcolor{black!15}\textbf{100.0} &  \cellcolor{black!15}\textbf{100.0} &                                88.9 &                                85.2 &                                81.5 &                                66.7 &                                59.3 &                                88.9 &                                40.7 &                                74.1 &                                59.3 \\
English - Spanish    &  25 &            \cellcolor{black!15}92.0 &            \cellcolor{black!15}88.0 &            \cellcolor{black!15}88.0 &   \cellcolor{black!15}\textbf{96.0} &                                76.0 &            \cellcolor{black!15}92.0 &            \cellcolor{black!15}92.0 &            \cellcolor{black!15}88.0 &            \cellcolor{black!15}92.0 &                                84.0 &                                72.0 &                                84.0 \\
\bottomrule
\end{tabular}
\end{table}


==> generated/generated_lang_pairs_counts.tex <==
\begin{table}
\centering
\caption{}
\label{tab:lang_pairs_counts}
\begin{tabular}{lrrlrrlrr}
\toprule
        Language pair &  Sys. &  Size &         Language pair &  Sys. &  Size &         Language pair &  Sys. &  Size \\
\midrule
     English - French &   145 &  1034 &       English - Hindi &    58 &   540 &   English - Ukrainian &    25 &   988 \\
     English - German &   139 &  2544 &      Polish - English &    57 &  1229 &      English - Slovak &    25 &  1776 \\
     French - English &   131 &  1119 &  Portuguese - English &    57 &   878 &       English - Irish &    24 &   463 \\
     German - English &   122 &  1212 &     Swedish - English &    57 &  1116 &     English - Persian &    24 &   510 \\
   Japanese - English &    78 &   925 &      English - Arabic &    56 &  1054 &      Slovak - English &    23 &  1476 \\
    Chinese - English &    74 &  1029 &      Korean - English &    56 &  1462 &       Greek - English &    23 &  1526 \\
    Italian - English &    71 &  1156 &       Czech - English &    55 &  1105 &    English - Croatian &    22 &  1625 \\
 English - Portuguese &    70 &  1679 &   English - Hungarian &    55 &  1018 &       English - Welsh &    22 &   497 \\
   English - Japanese &    67 &   998 &      English - Korean &    55 &   550 &   English - Norwegian &    22 &  1533 \\
    English - Swedish &    66 &  1219 &     English - Turkish &    55 &  1043 &      English - Hebrew &    22 &   940 \\
    English - Chinese &    65 &  2443 &        English - Thai &    54 &   510 &  English - Vietnamese &    20 &  1857 \\
     English - Danish &    64 &  1186 &       Hindi - English &    54 &   816 &       Welsh - English &    20 &  1686 \\
    English - Italian &    64 &  1505 &     Turkish - English &    54 &  1037 &  Vietnamese - English &    20 &  1697 \\
     English - Polish &    64 &  1188 &      Danish - English &    52 &   986 &     Catalan - English &    20 &   928 \\
    Spanish - English &    64 &  1223 &     English - Russian &    49 &  1159 &        English - Urdu &    18 &   448 \\
      Dutch - English &    63 &   927 &     Russian - English &    44 &   736 &     English - Finnish &    17 &  1802 \\
      English - Dutch &    61 &   991 &        Thai - English &    39 &   457 &       Tamil - English &    16 &   834 \\
 English - Indonesian &    61 &   948 &     English - Catalan &    30 &   981 &  English - Lithuanian &    16 &  1997 \\
 Indonesian - English &    60 &   703 &      Hebrew - English &    28 &   870 &  Lithuanian - English &    16 &  1997 \\
      English - Czech &    59 &  1329 &    English - Romanian &    27 &  1056 &     English - Maltese &    16 &   489 \\
     Arabic - English &    59 &  2674 &    Romanian - English &    27 &  1094 &   English - Kiswahili &    16 &   457 \\
    English - Spanish &    58 &  1172 &       English - Greek &    27 &  1936 &                       &       &       \\
  Hungarian - English &    58 &   976 &     Persian - English &    26 &  1372 &                       &       &       \\
\bottomrule
\end{tabular}
\end{table}


==> generated/generated_scenarios_accuracies.tex <==
\begin{table}
\centering
\caption{}
\label{tab:scenarios_accuracies}
\begin{tabular}{llllllll}
\toprule
{} &                         Everything &                            Into EN &                            From EN &                          Non Latin &                          Logograms &                            Non WMT &                             Speech \\
\midrule
n         &                               1717 &                                922 &                                768 &                                131 &                                 44 &                                484 &                                 78 \\
COMET     &  \cellcolor{black!15}\textbf{96.5} &  \cellcolor{black!15}\textbf{95.3} &  \cellcolor{black!15}\textbf{98.3} &  \cellcolor{black!15}\textbf{96.2} &  \cellcolor{black!15}\textbf{90.9} &  \cellcolor{black!15}\textbf{97.3} &  \cellcolor{black!15}\textbf{93.6} \\
COMET-src &                               95.3 &                               93.5 &           \cellcolor{black!15}97.7 &           \cellcolor{black!15}95.4 &           \cellcolor{black!15}88.6 &           \cellcolor{black!15}96.7 &  \cellcolor{black!15}\textbf{93.6} \\
Prism     &                               94.5 &                               92.2 &           \cellcolor{black!15}98.2 &  \cellcolor{black!15}\textbf{96.2} &  \cellcolor{black!15}\textbf{90.9} &           \cellcolor{black!15}96.9 &                               83.3 \\
BLEURT    &                               93.8 &                               93.8 &                               95.1 &           \cellcolor{black!15}93.1 &           \cellcolor{black!15}84.1 &                               94.6 &           \cellcolor{black!15}89.7 \\
ESIM      &                               92.9 &                               90.6 &                               96.6 &           \cellcolor{black!15}93.9 &           \cellcolor{black!15}86.4 &                               94.8 &                               76.9 \\
BERTScore &                               92.2 &                               91.2 &                               94.1 &           \cellcolor{black!15}95.4 &           \cellcolor{black!15}88.6 &                               92.8 &                               71.8 \\
ChrF      &                               89.5 &                               88.7 &                               91.0 &           \cellcolor{black!15}95.4 &           \cellcolor{black!15}88.6 &                               89.7 &                               57.7 \\
TER       &                               89.2 &                               87.6 &                               91.7 &                               90.1 &                               72.7 &                               90.9 &                               70.5 \\
CharacTER &                               88.6 &                               86.4 &                               91.7 &                               88.5 &                               70.5 &                               91.9 &                               69.2 \\
BLEU      &                               88.2 &                               86.9 &                               90.5 &           \cellcolor{black!15}92.4 &           \cellcolor{black!15}79.5 &                               89.9 &                               61.5 \\
Prism-src &                               85.3 &                               80.8 &                               91.4 &                               84.0 &                               65.9 &                               91.7 &                               84.6 \\
EED       &                               79.4 &                               75.1 &                               84.8 &                               82.4 &                               54.5 &                               83.1 &                               60.3 \\
\bottomrule
\end{tabular}
\end{table}


==> generated/generated_statitical_tests.tex <==
\begin{table}
\centering
\caption{}
\label{tab:statitical_tests}
\begin{tabular}{lllllll}
\toprule
{} &        No test &          Boot. &       Error II. & Error II. perc &                n &           boot n \\
\midrule
COMET     &  \textbf{83.4} &  \textbf{95.1} &           204.0 &           17.3 &  \textbf{3344.0} &           2093.0 \\
ESIM      &           78.7 &           95.0 &             7.0 &           20.6 &  \textbf{3344.0} &             20.0 \\
COMET-src &           83.2 &           94.2 &           242.0 &           19.4 &  \textbf{3344.0} &           2023.0 \\
BLEURT    &           80.0 &           92.0 &           349.0 &           25.4 &  \textbf{3344.0} &           1952.0 \\
Prism     &           80.6 &           91.3 &           200.0 &           18.3 &  \textbf{3344.0} &  \textbf{2231.0} \\
BERTScore &           78.3 &           87.9 &           244.0 &           20.9 &  \textbf{3344.0} &           2154.0 \\
ChrF      &           75.6 &           85.4 &           350.0 &           27.3 &  \textbf{3344.0} &           2044.0 \\
BLEU      &           74.6 &           83.4 &  \textbf{378.0} &           27.4 &  \textbf{3344.0} &           1942.0 \\
Prism-src &           73.4 &           81.5 &           325.0 &  \textbf{29.4} &  \textbf{3344.0} &           2219.0 \\
\bottomrule
\end{tabular}
\end{table}


==> generated/generated_system_level_alphas.tex <==
\begin{table}
\centering
\caption{}
\label{tab:system_level_description}
\begin{tabular}{llllll}
\toprule
{} &                                All &                               0.05 &                               0.01 &                              0.001 &                             Within \\
\midrule
n         &                               3344 &                               1717 &                               1420 &                               1176 &                                541 \\
COMET     &  \cellcolor{black!15}\textbf{83.4} &  \cellcolor{black!15}\textbf{96.5} &  \cellcolor{black!15}\textbf{98.7} &  \cellcolor{black!15}\textbf{99.2} &  \cellcolor{black!15}\textbf{90.6} \\
COMET-src &           \cellcolor{black!15}83.2 &                               95.3 &                               97.4 &                               98.1 &           \cellcolor{black!15}89.1 \\
Prism     &                               80.6 &                               94.5 &                               97.0 &                               98.3 &                               86.3 \\
BLEURT    &                               80.0 &                               93.8 &                               95.6 &                               98.2 &                               84.1 \\
ESIM      &                               78.7 &                               92.9 &                               95.6 &                               97.5 &                               82.8 \\
BERTScore &                               78.3 &                               92.2 &                               95.2 &                               97.4 &                               81.0 \\
ChrF      &                               75.6 &                               89.5 &                               93.5 &                               96.2 &                               75.0 \\
TER       &                               75.6 &                               89.2 &                               93.0 &                               96.2 &                               73.9 \\
CharacTER &                               74.9 &                               88.6 &                               91.9 &                               95.2 &                               74.1 \\
BLEU      &                               74.6 &                               88.2 &                               91.7 &                               94.6 &                               74.3 \\
Prism-src &                               73.4 &                               85.3 &                               87.6 &                               88.9 &                               77.4 \\
EED       &                               68.8 &                               79.4 &                               82.4 &                               84.6 &                               68.2 \\
\bottomrule
\end{tabular}
\end{table}


==> generated/generated_system_level_alphas_variants.tex <==
\begin{table}
\centering
\caption{}
\label{tab:system_level_description}
\begin{tabular}{llllll}
\toprule
{} &                                  All &                                 0.05 &                               Within &        Spearman &         Pearson \\
\midrule
n            &                                 3344 &                                 1717 &                                  541 &            3347 &            3347 \\
COMET        &  \cellcolor{black!15}\textbf{83.400} &  \cellcolor{black!15}\textbf{96.500} &  \cellcolor{black!15}\textbf{90.600} &  \textbf{0.879} &  \textbf{0.919} \\
COMET-src    &           \cellcolor{black!15}83.200 &                               95.300 &           \cellcolor{black!15}89.100 &           0.824 &           0.855 \\
Prism        &                               80.600 &                               94.500 &                               86.300 &           0.827 &           0.839 \\
BLEURT-large &                               80.100 &                               94.400 &                               85.400 &           0.808 &           0.748 \\
BLEURT       &                               80.000 &                               93.800 &                               84.100 &           0.787 &           0.729 \\
ESIM         &                               78.700 &                               92.900 &                               82.800 &           0.780 &           0.835 \\
BERTScore    &                               78.300 &                               92.200 &                               81.000 &           0.772 &           0.824 \\
ChrF         &                               75.600 &                               89.500 &                               75.000 &           0.716 &           0.739 \\
TER          &                               75.600 &                               89.200 &                               73.900 &           0.708 &           0.321 \\
CharacTER    &                               74.900 &                               88.600 &                               74.100 &           0.700 &           0.757 \\
BLEU         &                               74.600 &                               88.200 &                               74.300 &           0.661 &           0.640 \\
Prism-src    &                               73.400 &                               85.300 &                               77.400 &           0.661 &           0.631 \\
EED          &                               68.800 &                               79.400 &                               68.200 &           0.531 &           0.541 \\
\bottomrule
\end{tabular}
\end{table}

